Diffusion probabilistic modeling of protein backbones in 3D for the motif-scaffolding problem

Construction of a scaffold structure that supports a desired motif, conferring protein function, shows promise for the design of vaccines and enzymes. But a general solution to this motif-scaffolding problem remains open. Current machine-learning techniques for scaffold design are either limited to unrealistically small scaffolds (up to length 20) or struggle to produce multiple diverse scaffolds. We propose to learn a distribution over diverse and longer protein backbone structures via an E(3)-equivariant graph neural network. We develop SMCDiff to efficiently sample scaffolds from this distribution conditioned on a given motif; our algorithm is the first to theoretically guarantee conditional samples from a diffusion model in the large-compute limit. We evaluate our designed backbones by how well they align with AlphaFold2-predicted structures. We show that our method can (1) sample scaffolds up to 80 residues and (2) achieve structurally diverse scaffolds for a fixed motif.

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See computational experiments in \cref{sec:experiments}.}
  \item Did you describe the limitations of your work?
    \answerYes{See discussion in \cref{sec:discussion}. Other dedicated subsections in main and supplementary text discuss specific limitations with supporting evidence.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Our work advances protein engineering methodology which may have potential negative societal impact by advancing biotechnology. See discussion in \cref{sec:discussion}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{Propositions in the main text in \cref{sec:conditional_sampling} and supplementary specify all assumptions.}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{See \cref{sec:motif_scaffolding_formulation}.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See \cref{sec:experiments}. Code will be available on github with directions of obtaining the data.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See \cref{sec:data} and \cref{sec:training}}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{Our limited computational resources prohibited running AlphaFold2 for evaluation and obtaining enough data for error bars.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See \cref{sec:training}}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See references.}
  \item Did you mention the license of the assets?
    \answerYes{They are mentioned when necessary.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}



==> data.tex <==

For training, we restrict the data to single chain proteins (monomers) found in PDB and lengths below 128 residues. All structures with >5\AA{} resolution were removed. This amounted to 592 proteins. Next we performed self-consistency calculations over this training set to understand its \scRMSD{} distribution (see \cref{fig:train_filter}).
The distribution has a peak at <1\AA{} \scRMSD{} and a long tail past 1\AA. Examples that achieve >2\AA{} \scRMSD{} start to become unreliable to train with when the ground truth backbone cannot be recapitulated by AF2 with high accuracy.
% High \scRMSD{} for natural proteins may be explained due to  "marginally stable" hypothesis \cite{taverna2002proteins}. 
Training on non-designable proteins would give the model the incorrect inductive bias.
Therefore, we filtered out all proteins with >2\AA{} \scRMSD{} using \texttt{TM-align} which amounted to 433 proteins. A limitation of our set-up is the small amount of training data. Many monomers in PDB are larger than 128 residues but scaling \modelname \ to proteins larger than 128 proved to be challenging and is a direction for future work.
